A Timed Calculus for Mobile Ad Hoc Networks

We develop a timed calculus for Mobile Ad Hoc Networks embodying the peculiarities of local broadcast, node mobility and communication interference. We present a Reduction Semantics and a Labelled Transition Semantics and prove the equivalence between them. We then apply our calculus to model and study some MAC-layer protocols with special emphasis on node mobility and communication interference. A main purpose of the semantics is to describe the various forms of interference while nodes change their locations in the network. Such interference only occurs when a node is simultaneously reached by more than one ongoing transmission over the same channel.

==> eptcsdata.tex <==
\providecommand{\firstpage}{118}
\providecommand{\publicationstatus}{C.\ Artho and P.C.\ \"Olveczky (Eds.): FTSCS 2012\\
EPTCS 105, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.105.9}{10.4204/EPTCS.105.9}}
\pdfoutput=1

